Unit Invariance as a Unifying Principle of Physics

A basic principle of physics is the freedom to locally choose any unit system when describing physical quantities. Its implementation amounts to treating Weyl invariance as a fundamental symmetry of all physical theories. In this thesis, we study the consequences of this "unit invariance" principle and find that it is a unifying one. Unit invariance is achieved by introducing a gauge field called the scale, designed to measure how unit systems vary from point to point. In fact, by a uniform and simple Weyl invariant coupling of scale and matter fields, we unify massless, massive, and partially massless excitations. As a consequence, masses now dictate the response of physical quantities to changes of scale. This response is calibrated by certain "tractor Weyl weights". Reality of these weights yield Breitenlohner-Freedman stability bounds in anti de Sitter spaces. Another valuable outcome of our approach is a general mechanism for constructing conformally invariant theories. In particular, we provide direct derivations of the novel Weyl invariant Deser--Nepomechie vector and spin three-half theories as well as new higher spin generalizations thereof. To construct these theories, a "tractor calculus" coming from conformal geometry is employed, which keeps manifest Weyl invariance at all stages. In fact, our approach replaces the usual Riemannian geometry description of physics with a conformal geometry one. Within the same framework, we also give a description of fermionic and interacting supersymmetric theories which again unifies massless and massive excitations.

==> Abstract/abstract.tex <==
{\singlespacing
   \begin{flushright}
      Abrar Shaukat \\
      March 2009 \\
      Physics \\
   \end{flushright}
}

\bigskip
\doublespacing
\begin{center}
    Unit Invariance as a Unifying Principle of Physics\\
    \underline{\bf Abstract}
\end{center}

A basic principle of physics is the freedom to locally choose any unit system when describing physical quantities.  Its implementation amounts to treating Weyl invariance as a fundamental symmetry of all physical theories.  In this thesis, we study the consequences of this ``unit invariance" principle and find that it is a unifying one.  Unit invariance is achieved by introducing a gauge field called the scale, designed to measure how unit systems vary from point to point.  In fact, by a uniform and simple Weyl invariant coupling of scale and matter fields, we unify massless, massive, and partially massless excitations.  
As a consequence, masses now dictate the response of physical quantities to changes of scale.  This response is calibrated by certain ``tractor Weyl weights".  Reality of these weights yield Breitenlohner-Freedman stability bounds in anti de Sitter spaces.  Another valuable outcome of our approach is a general mechanism for constructing conformally invariant theories.  In particular, we provide direct derivations of the novel Weyl invariant Deser--Nepomechie vector and spin three-half theories as well as new higher spin generalizations thereof.  To construct these theories, a ``tractor calculus" coming from conformal geometry is employed, which keeps manifest Weyl invariance at all stages.   In fact, our approach replaces the usual Riemannian geometry description of physics with a conformal geometry one.
Within the same framework, we also give a description of fermionic and interacting supersymmetric theories which again unifies massless and massive excitations. 
